CREAM: Comparison-Based Reference-Free ELO-Ranked Automatic Evaluation for Meeting Summarization

Large Language Models (LLMs) have spurred interest in automatic evaluation methods for summarization, offering a faster, more cost-effective alternative to human evaluation. However, existing methods often fall short when applied to complex tasks like long-context summarizations and dialogue-based meeting summarizations. In this paper, we introduce CREAM (Comparison-Based Reference-Free Elo-Ranked Automatic Evaluation for Meeting Summarization), a novel framework that addresses the unique challenges of evaluating meeting summaries. CREAM leverages a combination of chain-of-thought reasoning and key facts alignment to assess conciseness and completeness of model-generated summaries without requiring reference. By employing an ELO ranking system, our approach provides a robust mechanism for comparing the quality of different models or prompt configurations.

==> table/REALSum_completeness.tex <==
\begin{table}[t]
\resizebox{\textwidth}{!}{%
\begin{tabular}{lllll}
\textbf{human-annotated key-fact}      & \textbf{human-annotated key-fact(\%)} & \textbf{machine-annotated key-facts (GPT4, two steps) (\%)} & \textbf{\begin{tabular}[c]{@{}l@{}}machine-annotated key-facts\\ (GPT4, one step, use summary)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}l@{}}machine-annotated key-facts\\ (GPT4, one step, use transcript)\end{tabular}} \\
unilm\_out\_v2                         & 48.2                                  & 45.7                                                        & 97.7                                                                                                         & 51.7                                                                                                            \\
t5\_out\_large                         & 46.6                                  & 42.0                                                        & 97.3                                                                                                         & 46.5                                                                                                            \\
fast\_abs\_rl\_out\_rerank             & 42.3                                  & 40.1                                                        & 95.8                                                                                                         & 45.8                                                                                                            \\
banditsumm\_out  \%                    & 49.8                                  & 44.3                                                        & 97.5                                                                                                         & 63.6                                                                                                            \\
ptr\_generator\_out\_pointer\_gen\_cov & 41.0                                  & 37.2                                                        & 97.1                                                                                                         & 51.4                                                                                                            \\
presumm\_out\_trans\_abs               & 42.3                                  & 39.4                                                        & 98.8                                                                                                         & 51.8                                                                                                            \\
semsim\_out                            & 59.6                                  & 55.8                                                        & 97.3                                                                                                         & 58.0                                                                                                            \\
presumm\_out\_ext\_abs                 & 45.1                                  & 41.8                                                        & 97.7                                                                                                         & 50.0                                                                                                            \\
presumm\_out\_abs                      & 43.7                                  & 40.8                                                        & 98.3                                                                                                         & 47.5                                                                                                            \\
neusumm\_out                           & 52.5                                  & 49.3                                                        & 98.0                                                                                                         & 65.8                                                                                                            \\
unilm\_out\_v1                         & 47.0                                  & 43.5                                                        & 97.4                                                                                                         & 48.2                                                                                                            \\
t5\_out\_base                          & 47.3                                  & 44.4                                                        & 96.4                                                                                                         & 45.9                                                                                                            \\
bottom\_up\_out                        & 37.6                                  & 33.1                                                        & 94.9                                                                                                         & 42.2                                                                                                            \\
t5\_out\_11B                           & 48.0                                  & 43.4                                                        & 96.2                                                                                                         & 47.7                                                                                                            \\
bart\_out\_abs                         & 53.0                                  & 49.2                                                        & 98.3                                                                                                         & 51.6                                                                                                            \\
two\_stage\_rl\_out                    & 44.6                                  & 41.4                                                        & 97.3                                                                                                         & 45.8                                                                                                            \\
matchsumm\_out                         & 53.3                                  & 48.6                                                        & 98.5                                                                                                         & 59.2                                                                                                            \\
heter\_graph\_out                      & 51.9                                  & 46.8                                                        & 98.0                                                                                                         & 56.9                                                                                                            \\
bart\_out\_ext                         & 58.0                                  & 55.2                                                        & 97.7                                                                                                         & 60.0                                                                                                            \\
refresh\_out                           & 61.3                                  & 57.9                                                        & 99.0                                                                                                         & 78.6                                                                                                            \\
pnbert\_out\_bert\_tf\_sl              & 52.6                                  & 46.3                                                        & 98.1                                                                                                         & 64.1                                                                                                            \\
pnbert\_out\_bert\_lstm\_pn            & 52.3                                  & 48.5                                                        & 97.5                                                                                                         & 61.3                                                                                                            \\
pnbert\_out\_bert\_tf\_pn              & 50.0                                  & 47.2                                                        & 98.4                                                                                                         & 65.7                                                                                                            \\
pnbert\_out\_bert\_lstm\_pn\_rl        & 52.7                                  & 48.8                                                        & 98.0                                                                                                         & 70.3                                                                                                            \\
pnbert\_out\_lstm\_pn\_rl              & 51.5                                  & 49.0                                                        & 97.7                                                                                                         & 66.5                                                                                                           
\end{tabular}%
}
\end{table}

==> table/completeness_baseline.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
\begin{table*}[ht]
\centering
\resizebox{0.6\textwidth}{!}{%
\begin{tabular}{ccccccc}
\hline
Max\# keyfacts &
  \begin{tabular}[c]{@{}c@{}}Summary\\ model\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Human summary\\ (GPT4o)\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Machine summary\\ (GPT4o)\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Transcript\\ (GPT4o)\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Transcript\\ (GPT4)\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Transcript\\ (GPT3.5)\end{tabular} \\ \hline
\multirow{3}{*}{16} & GPT3.5 & 56.2\%          & 100.0\% & 89.7\%          & 99.3\%          & \textbf{99.9\%} \\ \cline{2-7} 
                    & GPT4   & 57.9\%          & 100.0\% & 88.5\%          & 99.0\%          & 99.8\%          \\ \cline{2-7} 
                    & GPT4o  & \textbf{77.9\%} & 100.0\% & \textbf{98.9\%} & \textbf{99.9\%} & 99.8\%          \\ \hline
\multirow{3}{*}{30} & GPT3.5 & 54.8\%          & 100.0\% & 82.5\%          & 99.4\%          & \textbf{99.9\%} \\ \cline{2-7} 
                    & GPT4   & 55.6\%          & 100.0\% & 81.2\%          & 99.4\%          & 98.9\%          \\ \cline{2-7} 
                    & GPT4o  & \textbf{76.9\%} & 100.0\% & \textbf{98.1\%} & \textbf{99.9\%} & 99.7\%          \\ \hline
\end{tabular}%
}
\caption{Completeness score calculated using different type of source text to extract key facts, using different set up of the model (Same prompt, only differ in model type and in max number of key facts allowed). Max\# keyfacts column notes the max number of key facts extracted set by prompt. For example, 56.2\% means GPT4o models extracted key-facts from human summary used to evaluate the summary generated by GPT 3.5, when max number of key facts allowed are 16. "Human Summary" column is the gold standard baseline.}
\label{tab:completeness-baseline-table}
\end{table*}

==> table/cream-raw-comp.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
\begin{table}[t]
\centering
\resizebox{0.7\columnwidth}{!}{%
\begin{tabular}{lllll}
\multicolumn{5}{c}{\textbf{Completeness}}                                           \\ \hline
\#kf                & \textbf{VS} & \textbf{GPT3.5} & \textbf{GPT4}   & \textbf{GPT4o} \\ \hline
\multirow{3}{*}{16} & GPT3.5      & -               & \textbf{78.8\%} & 84.2\%         \\
                    & GPT4        & 76.6\%          & \textbf{-}      & 86.6\%         \\
                    & GPT4o       & \textbf{92.1\%} & \textbf{94.0\%} & -              \\ \hline
\multirow{3}{*}{30} & GPT3.5      & -               & \textbf{80.7\%} & 82.2\%         \\
                    & GPT4        & 80.0\%          & -               & 86.3\%         \\
                    & GPT4o       & \textbf{94.9\%} & \textbf{95.5\%} & -             
\end{tabular}%
}
\caption{Raw completeness score on QMSum. machine-annotated key facts (GPT-4o, one step, use both), \# kf denotes max number of key facts set}
\label{tab:raw-cream-completness}
\end{table}

==> table/cream-raw-conc.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
\begin{table}[t]
\centering
\resizebox{0.7\columnwidth}{!}{%
\begin{tabular}{lllll}
\multicolumn{5}{c}{\textbf{Conciseness}}                                           \\ \hline
\#kf                & VS     & GPT3.5          & GPT4            & GPT4o           \\ \hline
\multirow{3}{*}{16} & GPT3.5 & -               & \textbf{90.0\%} & \textbf{87.5\%} \\
                    & GPT4   & \textbf{93.6\%} & \textbf{-}      & \textbf{92.1\%} \\
                    & GPT4o  & \textbf{67.3\%} & \textbf{68.4\%} & -               \\ \hline
\multirow{3}{*}{30} & GPT3.5 & -               & 99.1\%          & \textbf{96.4\%} \\
                    & GPT4   & \textbf{99.4\%} & \textbf{-}      & \textbf{95.9\%} \\
                    & GPT4o  & 89.7\%          & 88.6\%          & -              
\end{tabular}%
}
\caption{Raw conciseness score on QMSum.}
\label{tab:raw-cream-conc}
\end{table}

==> table/zoom_keyfacts_ablation_4o.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table}[t]
\resizebox{0.5\textwidth}{!}{%
\begin{tabular}{lllllllll}
\begin{tabular}[c]{@{}l@{}}\#of key facts\\ (OneStep,\\ key fact from Transcript\\ + focus on middle (2)\end{tabular} & 16    & 20   & 30             & 40    & 50    & 60    & 70   & 100   \\
summary\_0\_short                                                                                                     & 98.3  & 98.5 & 92.4           & 96.0  & 87.5  & 81.6  & 92.9 & 97.9  \\
summary\_0\_long                                                                                                      & 100.0 & 98.5 & 91.7           & 91.4  & 81.6  & 87.3  & 87.6 & 93.8  \\
average length of key facts extracted                                                                                 & 15.8  & 19.7 & \textbf{26.54} & 26.13 & 18.58 & 20.05 & 22.3 & 22.05 \\
failure case: wrong key facts                                                                                         & 0     & 0    & 1              & 1     & 4     & 4     & 3    & 1     \\
score without failure cases: summary\_0\_short                                                                        & 98.3  & 98.5 & 92.4           & 96.0  & 92.1  & 90.6  & 97.8 & 97.9  \\
score without failure cases: summary\_0\_long                                                                         & 100.0 & 98.5 & 96.5           & 96.3  & 96.1  & 97.0  & 97.4 & 98.7  \\
score without failure cases: avg\_len                                                                                 & 15.8  & 19.7 & \textbf{27}    & 26.6  & 19.6  & 21.3  & 23.4 & 22.4 
\end{tabular}%
}
\caption{Explore \# of key fact and its affect (GPT4o)}
\label{tab:my-table}
\end{table}



